Future memories are not needed for large classes of POMDPs

Optimal policies for partially observed Markov decision processes (POMDPs) are history-dependent: Decisions are made based on the entire history of observation. Memoryless policies, which take decisions based on the last observation only, are generally considered useless in the literature because we can construct POMDP instances for which optimal memoryless policies are arbitrarily worse than history-dependent ones. Our purpose is to challenge this belief. We show that optimal memoryless policies can be computed efficiently using mixed integer linear programming (MILP), and perform reasonably well on a wide range of instances from the literature. When strengthened with valid inequalities, the linear relaxation of this MILP provides high quality upper-bounds on the value of an optimal history dependent policy. Furthermore, when used with a finite horizon POMDP problem with memoryless policies as rolling optimization problem, a model predictive control approach leads to an efficient history-dependent policy, which we call the short memory in the future (SMF) policy. Basically, the SMF policy leverages these memoryless policies to build an approximation of the Bellman value function. Numerical experiments show the efficiency of our approach on benchmark instances from the literature.

==> sections/appCounteExample.tex <==
%!TEX root=../generalPomdp.tex

\section{Example where $v_{\rmSMF}^{T}(\bfb)$ is arbitrarily worse than $v^*(\bfb)$}
\label{app:counter_example}


In this section, we describe a POMDP instance for which the value of SMF policy, for any finite hoirzon $T$, can be arbitrarly worse than the optimal POMDP value.

\inlVC{Je ne me souviens plus trop comment on prouve que notre contre-exemple est bien un contre-exemple. J'ai gardé ce que tu avais écrit, mais je ne me souviens plus de l'argument crucial qui nous assurait ça.}

==> sections/conclusion.tex <==
%!TEX root=../generalPomdp.tex
\section{Conclusion}
\label{sec:conclusion}



